Approximating Human Judgment of Generated Image Quality

Generative models have made immense progress in recent years, particularly in their ability to generate high quality images. However, that quality has been difficult to evaluate rigorously, with evaluation dominated by heuristic approaches that do not correlate well with human judgment, such as the Inception Score and Fr\'echet Inception Distance. Real human labels have also been used in evaluation, but are inefficient and expensive to collect for each image. Here, we present a novel method to automatically evaluate images based on their quality as perceived by humans. By not only generating image embeddings from Inception network activations and comparing them to the activations for real images, of which other methods perform a variant, but also regressing the activation statistics to match gold standard human labels, we demonstrate 66% accuracy in predicting human scores of image realism, matching the human inter-rater agreement rate. Our approach also generalizes across generative models, suggesting the potential for capturing a model-agnostic measure of image quality. We open source our dataset of human labels for the advancement of research and techniques in this area.

==> others.tex <==
\section{Biologically Plausible Deep Learning}
\subsection{Over-Parameterization}
\citep{hinton2016backpropagation}
One thing deep learning could learn from the brain is that there is very little need to limit model parameter. The brain has about $10^{14}$ synapses, while the entire human life is only about $10^9$ seconds. Therefore, a powerful regularization is highly important. A very successful strategy is drop out. There are two ways to do this with similar results
\begin{enumerate}
\item Set the value of a unit to zero with prob $1/2$
\item Multiply activation of the unit by a Gaussian noise with same stddiv as activation 
\end{enumerate}
The success of this shows that representations are highly redundant, noisy, which prevents over-fitting. Therefore the spike based Poisson process activations may be beneficial rather than harmful.

\subsection{STDP as Back Propagation}
\citep{hinton2016backpropagation} The key objection to backprop in the brain is the difficulty of computing backward gradients. One possible implementation is
\begin{itemize}
\item $y_i$ represents post synaptic activity
\item $\dot{y_i}$ represents error derivative w.r.t. pre-synaptic total activity  $\partial E/\partial x_i$
\end{itemize}
The STDP (Stochastic temporal dynamic plasticity) corresponds to an update rule of 
\[ \Delta w_ij \propto y_{pre} \dot{y}_{post} \]
and this would be the same as backprop if 
\[ \dot{y}_{post} = \partial E/\partial x_{post} \]
which can be achieved by a simple implementation. For the top layer let $d_j$ be target
\[ y_j(t) = y_j(0) + t d_j - t y_j(0) \]
then
\[ \dot{y}_j(t) = d_j - y_j(0) = -\frac{\partial E}{\partial x_j} \]
where the last equality is true if loss is cross entropy.

For lower layers suppose we know $\dot{y}_j = \partial E/\partial x_j$ and $\dot{y}_k = \partial E/\partial x_k$, etc for upper layer, for lower layer neuron $x_i$, we can apply reciprocal connections
\[ x_i = w_{ji} y_j + w_{ki} y_k \]
and
\[ \dot{y}_i = (w_{ji}\dot{y}_j + w_{ki} \dot{y}_k) \frac{\partial y_i}{\partial x_i} \]
By the backprop principle this is equal to
\[ \dot{y}_i = \partial E/\partial x_i \]
But this assumes that the forward weights are copied to perform backward propagation. 
\citep{lillicrap2014random} actually shows that even when the backward weights are random we can still achieve performance comparable to backprop. 

Suppose rather than $\Delta y_l = W^T \Delta x_{l+1}$, we use a random matrix $B$ in place of $W^T$. It is discovered that during training $angle(W^T e, Be)$, where $e$ is upper layer error signal quickly drops from averaging to $90 \deg$ to much lower, which means that the error signals computed by the two methods quickly align. 

\myfigure[0.9]{plots/random-backprop}

\subsection{Predictive Coding Theory}
\begin{enumerate}
\item The survey \citep{huang2011predictive} claims that feedback connections in the brain carries predictions of lower layers, while feed forward connections propagate prediction errors. This is supported by various neural science experiments relating to vision, audition, hippo-campus path finding, etc. 
\item The paper \citep{rao1999predictive} proposes predictive coding as a method of maximizing likelihood of a generative model with respect to image input. 
\[ r^{l-1} = f(Ur^l) + n^{l-1} \]
where $n$ is Gaussian noise. The log likelihood looks like
\[ E_l = \frac{1}{\sigma_l^2} ||r^{l-1} - f(U^l r^l)||_2^2 + g(r^l) + h(U^l) \]
The gradient descent can be implemented by the following predictive estimator unit
\myfigure[0.9]{plots/predictive_estimator}
This architecture has been shown to learn early visual activation patterns and the end-stopping phenomenon, where response at a particular location is weakened if the pattern repeats spatially. 

\item In \citep{friston2005cortical,friston2003cortical}
The evidence supporting the hypothesis are
\begin{itemize}
\item The brain is organized as a hierarchy, distinguished by forward and backward connections
\item Brain areas are specialized and functions are localized. However an area may perform different functions depending on the context
\item Structural evidence suggest that forward connections are driving while backward connections are modulatory
\item Forward connections are faster (AMPA), while backward connections are slower (NMDA), suggesting that backward connections main states about the world while forward connections are transient
\item Backward connections are more numerous, more divergent (one point associates with a larger region), and spread across more layers
\end{itemize}

\end{enumerate}


\section{Misc}
\citep{cognitive_science_intro2010}There are five big questions in cognitive science and machine provides some tools for their resolution

\begin{table*}[h]
\centering
\begin{tabular}{p{0.4\textwidth} | p{0.4\textwidth}}
How do knowledge guide inductive learning from sparse, noisy data & Bayesian inference in probablistic generative models \\
\hline
What are the forms and contents of knowledge & probabilities over structured representations \\ \hline
How is knoeledge learned from experience & hierarchical probablistic models, with inference at every level of abstraction \\ \hline
How to balance flexibility with constraint & adaptive non-parametric models, such as CRP \\ \hline
How can inductive inference be made efficiently & approximate methods such as MCMC \\
\end{tabular}
\end{table*}

It is not possible by learning theory to generalize from a single example, but people still do it non-the-less (Why? TODO: find more detail on a proof of this statement from LT perspective)

\subsection{Computation rationality\citep{computational_rationality2015}}
Agents are often measured by their maximum expected utility (MEU). However, most optimization problems are hard and the agent must balance the amount of computational efforts used, since expected utility decreases with time taken to think.  The brain apparently applies such strategies. For example, regions of the prefrontal cortex are activated when people make decisions about the amount of cognitive efforts to put into a problem. This tradeoff is often manifest in model-based and model-free tradeoff. Model-based search/sampling/optimization is often expansive but flexible, while model-free caching is cheap, but generalize poorly to novel situations. When the experience is rather new, there is little caching to use, and the agent acts slower, relying more on model-based computation. Later the agent forms habits or reflexes, and acts faster. There is significant evidence that the brain performs meta-reasoning to decide how much to rely on either methods.

\subsection{Simulation for Physical Scene Understanding\citep{simulation_for_physical2013}}
 Proposes that humans are able to predict the progression of physical system (such as if a stack of blocks will fall) by a rough noisy (stochastic) simulation process. The model proposed match actual psychological data (of people's predictions) very well, in fact, much better than physical ground truth. This simulation process is also possible in a variety of predictive settings, and holds advantages over model-free approaches (such as supervised prediction). 

Idea: It seems reasonable that humans are able to predict through simulation. However can we learn the simulation parameters by observations? Maybe build a model that observes the motion of blocks and infer the presence of gravity, friction, etc by somehow back-prop against the simulation results (What the simulation should be vs. what the simulation turned out to be)

\subsection{The Large-Scale Structure of Semantic Networks\citep{semantic_network_structure2005}}
For a semantic network, for example, an associative network where subjects are asked to identify the first related word that comes to mind, or an meaning network, where two words are associated if they share a meaning, have statistical structures that differ greatly from random graphs with similar connection density.
\begin{enumerate}
\item Small-world property, where neighbors of a node are likely to be associated themselves. This can be measured the porportion of point pairs in the neighborhood that are connected. For semantic network this value is often orders of magnitude larger than random networks, suggesting clustered structure
\item Power-law property, where the probably a node taking degree $k$ satisfies
\[ P(k) \propto k^{-\gamma} \]
while a random network is more likely to demonstrate exponential distribution
\item Small and scale invariant width: the longest distance between one node to another is very small $\approx 5$
\end{enumerate}
One model for explaining these properties is the following graph generation process (For undirected case)
\begin{enumerate}
\item The network starts with $M$ nodes
\item A node is added, differentiating a existing node chosen with probability in proportion to its current degree (preferential attachment). By differntiation, the new node connects with $M$ randomly chosen nodes among the neighbors of the selected node
\end{enumerate}
$M$ is selected based on intended network sparsity. This process generates statistics very similar to those observed in real semantic networks
